A Bar-Natan homotopy type

A spatial refinement of Bar-Natan homology is given, that is, for any link diagram $D$ we construct a CW-spectrum $\mathcal{X}_{\mathit{BN}}(D)$ whose reduced cellular cochain complex gives the Bar-Natan complex of $D$. The stable homotopy type of $\mathcal{X}_{\mathit{BN}}(D)$ is a link invariant and is described as the wedge sum of the canonical cells. We conjecture that the quantum filtration of Bar-Natan homology also lifts to the spatial level, and that it leads us to a cohomotopical refinement of the $s$-invariant.

==> tikz-cd/XY-edge-labeling.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,138); %set diagram left start at 0, and has height of 138

%Shape: Circle [id:dp7242830239792952] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (25,55.24) .. controls (25,35.78) and (40.78,20) .. (60.24,20) .. controls (79.71,20) and (95.49,35.78) .. (95.49,55.24) .. controls (95.49,74.71) and (79.71,90.49) .. (60.24,90.49) .. controls (40.78,90.49) and (25,74.71) .. (25,55.24) -- cycle ;
%Straight Lines [id:da30041319840711733] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (35.77,30.77) -- (84.72,79.72) ;
%Straight Lines [id:da6742767751751203] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (84.49,31) -- (35.49,80) ;

%Shape: Circle [id:dp8798997476150507] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (152,54.24) .. controls (152,34.78) and (167.78,19) .. (187.24,19) .. controls (206.71,19) and (222.49,34.78) .. (222.49,54.24) .. controls (222.49,73.71) and (206.71,89.49) .. (187.24,89.49) .. controls (167.78,89.49) and (152,73.71) .. (152,54.24) -- cycle ;
%Straight Lines [id:da8313927112135109] 
\draw [color={rgb, 255:red, 23; green, 0; blue, 255 }  ,draw opacity=1 ]   (162.77,29.77) -- (211.72,78.72) ;
%Straight Lines [id:da9430918514892531] 
\draw [color={rgb, 255:red, 23; green, 0; blue, 255 }  ,draw opacity=1 ]   (211.49,30) -- (162.49,79) ;

%Shape: Circle [id:dp5949309486187376] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (312,54.55) .. controls (312,35.08) and (327.78,19.31) .. (347.24,19.31) .. controls (366.71,19.31) and (382.49,35.08) .. (382.49,54.55) .. controls (382.49,74.01) and (366.71,89.79) .. (347.24,89.79) .. controls (327.78,89.79) and (312,74.01) .. (312,54.55) -- cycle ;
%Straight Lines [id:da01584200437866856] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (322.77,30.07) -- (346.9,54.2) ;
%Straight Lines [id:da8930656695225742] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (347.38,54.41) -- (322.49,79.31) ;
%Straight Lines [id:da7422233615785512] 
\draw [color={rgb, 255:red, 23; green, 0; blue, 255 }  ,draw opacity=1 ]   (347.24,54.24) -- (371.72,78.72) ;
%Straight Lines [id:da969472501871585] 
\draw [color={rgb, 255:red, 23; green, 0; blue, 255 }  ,draw opacity=1 ]   (371.49,30) -- (347.38,54.11) ;


% Text Node
\draw (302,14.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (302,75.71) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (377,16.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (377,77.71) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (142,15.09) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (142,76.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (217,15.45) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (218,77.75) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,opacity=1 ]  {$Y$};
% Text Node
\draw (15,15.09) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (15,76.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (90,15.45) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (89,77.75) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$X$};
% Text Node
\draw (95,107.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {type (I)};
% Text Node
\draw (320,106.38) node [anchor=north west][inner sep=0.75pt]   [align=left] {type (II)};


\end{tikzpicture}

==> tikz-cd/handle-slide-cancel-1.tex <==
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZARgBoAGAXVJADcBDAGwFcYkQAKMgAnNO4DuAShABfUuky58hFACYK1Ok1bsu-HsLESQGbHgJE+AZiUMWbRJx4c+vIfy3jJ+mUTKma51VfXc-xA6CIs66UgayyApyZiqW1vy2-ORBAtwA1NwwAOQhOnrShijGpDFecWo2PIGOGVm5YkowUADm8ESgAGYAThAAtkh8IDgQSGQgjFhg8VD0cAAWzdpdvQOIQyNIcqE9-Vs0m4glE1Mzc4tQyyC7awAsB6OIAKw0k9PsswtLO6tjD0jGH57db-I40ABGMDAl0QAFpjOQgWsNo9bkjBqCXiBIdCkPDETobn9ho8nuiQSSAa9Th8IDgcEsIVCYQjySikFi3jM6QzLkzcUcCStgQpKYh7id3lZPhcrkSwWLOTTpedvpRREA
\begin{tikzcd}[row sep={1cm,between origins}, column sep={1.8cm,between origins}]
                                                       & {\x} \arrow[r, dashed] \arrow[lddd, "+"', red] \arrow[ddd, "+"', red, bend right=15] \arrow[ddd, "-", dotted, blue, bend left=15] \arrow[rdd, "\pm"', red] \arrow[rrdd, "\pm"', red, bend right=5] \arrow[rrdd, "\mp", dotted, blue, bend left=5]  & {\x'} \arrow[lddd, "-", blue] \arrow[rdd, "\mp", blue]    &                       \\
                                                       &                                                                                                                                                                        &                                         &                       \\
                                                       &                                                                                                                                                                        & {\bar{\y}} \arrow[r, dashed] & {\bar{\y}'} \\
{\y} \arrow[r, dashed] \arrow[rru, dashed] & {\y'} \arrow[rru, dashed]                                                                                                                                   &                                         &                      
\end{tikzcd}

==> tikz-cd/handle-slide-cancel-2.tex <==
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBoBGAXVJADcBDAGwFcYkQAdDgDxAF9S6TLnyEU5UsWp0mrdlwDGUCDn6CQGbHgJEyAZmkMWbRJw4BPNUK2iiAJlJ3Dsk2fMByKxuHaxyB1I0RnKmXNyeAtYiOuIUzsbyHEoqXprRfhIGQS6JyaqR3jYxyBJO2QmhScr50jBQAObwRKAAZgBOEAC2SGQgOBBIDjIVIADUXu1dPTT9SBIgjFhgrlD0cAAWdSA0m-RQSGDMjIw0G1gtqojEBZPdVzMDiACsNIvL7NU4Wzswe+yQ7xuHTuABYHkg9OUQmMJsCkAB2cGISELJYrFRffY-P6mAFsIFTRBDWaIABsrzRHzWm32BLu5L6jxRbxW1K2dMGSMRqPepk+3xAu32uII+PUtzmSLBPNZG3Z4rhzylFN5IH5WMFv2F4FFsMJvRJDOCrgAtHq7gamVDXOMaAAjGBgYUmvTXBWE+Yk7nG9jjDmIT1W4bQs3+y0Q+2O4Wu63sUOUPhAA
\begin{tikzcd}[row sep={2cm,between origins}, column sep={3cm,between origins}]
                                                                                                                                           & \x' \arrow[r, dashed] \arrow[dd, "+"', pos=.35, gray] \arrow[rdd, "-", gray, bend left=15] & \cdot \\
\x \arrow[dd, "+"] \arrow[ru, dashed] \arrow[r, no head, dotted] \arrow[rdd, "-", bend right=15] \arrow[rrd, "+", bend right=10, pos=.6] \arrow[rrd, "-", bend left=10, pos=.6, gray] &  \arrow[ru, no head, dotted]                        &                     \\
                                                                                                                                           & \cdot \arrow[r, no head, dotted]                         & \y                 \\
\cdot \arrow[r, dashed] \arrow[ru, no head, dotted]                                                                                           & \cdot \arrow[ru, dashed]                                 &                    
\end{tikzcd}
